Model-Guided Synthesis of Inductive Lemmas for FOL with Least Fixpoints

Recursively defined linked data structures embedded in a pointer-based heap and their properties are naturally expressed in pure first-order logic with least fixpoint definitions (FO+lfp) with background theories. Such logics, unlike pure first-order logic, do not admit even complete procedures. In this paper, we undertake a novel approach for synthesizing inductive hypotheses to prove validity in this logic. The idea is to utilize several kinds of finite first-order models as counterexamples that capture the non-provability and invalidity of formulas to guide the search for inductive hypotheses. We implement our procedures and evaluate them extensively over theorems involving heap data structures that require inductive proofs and demonstrate the effectiveness of our methodology.

==> table-app-theorems.tex <==
\begin{table*}
	\centering
	\caption{Theorems proven in constraint-based synthesis}
	\label{tbl:theorems-1}
	\small
	\begin{tabular}{| p{2.0cm} | p{10.0cm} |} 
		\hline
		\multicolumn{1}{|c|}{theorem name} & \multicolumn{1}{c|}{statement} \\ 
		\hhline{|==|}
		
		\hline dlist-list & dlst(x) $\Rightarrow$ (If(x $=$ nil, ret $=$ nil, ret $=$ nxt(x)) $\Rightarrow$ lst(ret)) \\
		\hline slist-list & slst(x) $\Rightarrow$ (If(x $=$ nil, ret $=$ nil, ret $=$ nxt(x)) $\Rightarrow$ lst(ret)) \\
		\hline sdlist-dlist & sdlst(x) $\Rightarrow$ (If(x $=$ nil, ret $=$ nil, ret $=$ nxt(x)) $\Rightarrow$ dlst(ret)) \\
		\hline sdlist-dlist-slist & sdlst(x) $\Rightarrow$ (If(x $=$ nil, ret $=$ nil, ret $=$ nxt(x)) $\Rightarrow$ dlst(ret) $\wedge$ slst(ret)) \\
		\hline listlen-list & listlen(x, l) $\Rightarrow$ (If(l $=$ 1, ret $=$ x, ret $=$ nxt(x)), list(x)) \\
		\hline even-list & even\textunderscore lst(x) $\Rightarrow$ (If(x $=$ nil, ret $=$ nil, ret $=$ nxt(x)) $\Rightarrow$ lst(ret)) \\
		\hline odd-list & odd\textunderscore lst(x) $\Rightarrow$ (If(x $=$ nil, ret $=$ nil, ret $=$ nxt(x)) $\Rightarrow$ lst(ret)) \\
		\hline list-even-or-odd & lst(x) $\Rightarrow$ (even\textunderscore lst(x) $\vee$ odd\textunderscore lst(x)) \\
		\hline lseg-list & lseg(x,y) $\Rightarrow$ (If(x $=$ nil, ret $=$ nil, ret $=$ nxt(x)) $\Rightarrow$ lst(ret)) \\
		\hline lseg-next & lseg(x,y) $\Rightarrow$ ((key(x) $\neq$ k $\wedge$ n(y) = z) $\Rightarrow$ lseg(x,z)) \\
		\hline lseg-next-dyn & lsegy(x) $\Rightarrow$ (key(x) $\neq$ k $\Rightarrow$ lsegz\textunderscore p(x)) \\
		\hline lseg-trans & lseg(x, y) $\Rightarrow$ (lst(y) $\wedge$ x $\neq$ c $\wedge$ nxt(y) $=$ z $\Rightarrow$ (lseg(x, z) $\wedge$ lst(z))) \\
		\hline lseg-trans2 & lseg(x, y) $\Rightarrow$ (key(x) $\neq$ k $\wedge$ lseg(y, z) $\Rightarrow$ lseg(x, z)) \\
		\hline lseg-ext & lseg(x, y) $\Rightarrow$ (key(x) $\neq$ k $\wedge$ lseg(x, z) $\Rightarrow$ lseg(y, z) $\vee$ lseg(z, y)) \\
		\hline lseg-nil-list & lseg(x, y) $\Rightarrow$ (If(x $=$ nil, ret $=$ nil, ret $=$ nxt(x)) $\Rightarrow$ (y $=$ nil $\Rightarrow$ list(ret))) \\
		\hline slseg-nil-slist & slseg(x, y) $\Rightarrow$ (If(x $=$ nil, ret $=$ nil, ret $=$ nxt(x)) $\Rightarrow$ (y $=$ nil $\Rightarrow$ slist(ret))) \\
		\hline list-hlist-list & lst(x) $\Rightarrow$ (key(x) $\neq$ k $\wedge$ y $\in$ hlst(x) $\Rightarrow$ lst(y)) \\
		\hline list-hlist-lseg & lst(x) $\Rightarrow$ (key(x) $\neq$ k $\wedge$ y $\in$ hlst(x) $\Rightarrow$ lseg(x,y)) \\
		\hline list-lseg-keys & lst(x) $\Rightarrow$ ((y $\neq$ nil $\wedge$ lseg(x,y) $\wedge$ key(y) $=$ k) $\Rightarrow$ k $\in$ keys(x)) \\
		\hline list-lseg-keys2 & lseg(x,y) $\Rightarrow$ ((x $\neq$ nil $\wedge$ y $\neq$ nil $\wedge$ lst(x) $\wedge$ key(y) $=$ k) $\Rightarrow$ k $\in$ keys(x)) \\
		\hline rlist-list & rlst(x) $\Rightarrow$ (If(x $=$ nil, ret $=$ nil, ret $=$ nxt(x)) $\Rightarrow$ lst(ret)) \\
		\hline rlist-black-height & rlst(x) $\Rightarrow$ (black(x) $\Rightarrow$ red\textunderscore height(x) $=$ black\textunderscore height(x)) \\
		\hline rlist-red-height & rlst(x) $\Rightarrow$ (red(x) $\Rightarrow$ red\textunderscore height(x) $=$ 1 + black\textunderscore height(x)) \\
		\hline cyclic-next & cyclic(x) $\Rightarrow$ cyclic(nxt(x)) \\
		\hline tree-dag & tree(x) $\Rightarrow$ (If(x $=$ nil, ret $=$ nil, ret $=$ lft(x)) $\Rightarrow$ dag(ret)) \\
		\hline
	\end{tabular}
\end{table*}
%\newpage
\begin{table*}
	\centering
	\caption{Theorems proven in constraint-based synthesis}
	\label{tbl:theorems-2}
	\small
	\begin{tabular}{| p{2.0cm} | p{10.0cm} |} 
		\hline
		\multicolumn{1}{|c|}{theorem name} & \multicolumn{1}{c|}{statement} \\ 
		\hhline{|==|}
		\hline bst-tree & bst(x) $\Rightarrow$ (If(x $=$ nil, ret $=$ nil, ret $=$ lft(x)) $\Rightarrow$ tree(ret)) \\
		\hline maxheap-dag & maxheap(x) $\Rightarrow$ (If(x $=$ nil, ret $=$ nil, ret $=$ lft(x)) $\Rightarrow$ dag(ret)) \\
		\hline maxheap-tree & maxheap(x) $\Rightarrow$ (If(x $=$ nil, ret $=$ nil, ret $=$ lft(x)) $\Rightarrow$ tree(ret)) \\
		\hline tree-p-tree & tree\textunderscore p(x) $\Rightarrow$ (parent(x) $=$ nil $\Rightarrow$ tree(x)) \\
		\hline tree-p-reach & tree\textunderscore p(x) $\Rightarrow$ (reach\textunderscore lr(x,y) $\Rightarrow$ tree\textunderscore p(y)) \\
		\hline tree-p-reach-tree & tree\textunderscore p(x) $\Rightarrow$ (parent(x) $=$ nil $\Rightarrow$ (reach\textunderscore lr(x,y) $\Rightarrow$ tree(y))) \\
		\hline tree-reach & reach(x,y) $\Rightarrow$ (tree(x) $\wedge$ key(x) $\neq$ k $\Rightarrow$ tree(y)) \\
		\hline tree-reach2 & tree(x) $\Rightarrow$ (reach(x,y) $\Rightarrow$ tree(y)) \\
		\hline dag-reach & reach(x,y) $\Rightarrow$ (dag(x) $\wedge$ key(x) $\neq$ k $\Rightarrow$ dag(y)) \\
		\hline dag-reach2 & dag(x) $\Rightarrow$ (reach(x,y) $\Rightarrow$ dag(y)) \\
		\hline reach-left-right & reach(x,y) $\Rightarrow$ (x $\neq$ nil $\wedge$ y $\neq$ nil $\wedge$ reach(lft(x), y) $\wedge$ reach(rght(x), z) $\Rightarrow$ y $\neq$ z) \\
		\hline bst-left & bst(x) $\Rightarrow$ ((x $\neq$ nil $\wedge$ k $\in$ keys(x) $\wedge$ k < key(x)) $\Rightarrow$ k $\in$ keys(lft(x))) \\
		\hline bst-right & bst(x) $\Rightarrow$ ((x $\neq$ nil $\wedge$ k $\in$ keys(x) $\wedge$ k > key(x)) $\Rightarrow$ k $\in$ keys(rght(x))) \\
		\hline bst-leftmost & ((x $\neq$ nil $\wedge$ key(x) $\neq$ k $\wedge$ y $=$ leftmost(x)) $\Rightarrow$ key(y) $=$ minr(x)) \\
		\hline bst-left-right & bst(x) $\Rightarrow$ ((x $\neq$ nil $\wedge$ y $\in$ hbst(lft(x)) $\wedge$ z $\in$ hbst(rght(x))) $\Rightarrow$ key(y) $\leq$ key(z)) \\
		\hline bst-maximal & bst(x) $\Rightarrow$ ((x $\neq$ nil y $\neq$ nil $\wedge$ rght(y) $\neq$ nil $\wedge$ y $\in$ hbst(x) $\wedge$ k $=$ maxr(x)) $\Rightarrow$ k $=$ maxr(lft(y))) \\
		\hline bst-minimal & bst(x) $\Rightarrow$ ((x $\neq$ nil y $\neq$ nil $\wedge$ lft(y) $\neq$ nil $\wedge$ y $\in$ hbst(x) $\wedge$ k $=$ minr(x)) $\Rightarrow$ k $=$ minr(lft(y))) \\
		\hline maxheap-htree-key & maxheap(x) $\Rightarrow$ (key(x) $\neq$ k $\Rightarrow$ (y $\in$ htree(x) $\Rightarrow$ key(y) $\leq$ key(x))) \\
		\hline maxheap-keys & maxheap(x) $\Rightarrow$ (lft(x) $\neq$ nil $\Rightarrow$ (k $\in$ keys(x) $\Rightarrow$ k $\leq$ key(x)) \\
		\hline
	\end{tabular}
\end{table*}
%\newpage
\begin{table*}
	\centering
	\caption{Theorems proven in constraint-based synthesis}
	\label{tbl:theorems-3}
	\small
	\begin{tabular}{| p{2.0cm} | p{10.0cm} |} 
		\hline
		\multicolumn{1}{|c|}{theorem name} & \multicolumn{1}{c|}{statement} \\ 
		\hhline{|==|}
		\hline reachability & {v1 = v2} \\ & while (v1 $\neq$ nil) do \\ &   v1 := n(v1); \\ &   if (v2 $\neq$ c) {v2 := n(v2)} \\ & endwhile \\ & {v2 = nil $\vee$ v2 = c} \\
		\hline reachability2 & {v1 = v2} \\ & while (v1 $\neq$ nil) do \\ &   v1 := n(v1); \\ &   v2 := n(v2) \\ & endwhile \\ & {v2 = nil} \\
		\hline reachability3 & {v1 = v2} \\ & while (v1 $\neq$ c) do \\ &   v1 := n(v1); \\ &   if (v2 $\neq$ c) {v2 := n(v2)} \\ & endwhile \\ & {v2 = nil $\vee$ v2 = c} \\
		\hline reachability4 & {v1 = v2} \\ & while (v1 $\neq$ c) do \\ &   v1 := n(v1); \\ &   v2 := n(v2) \\ & endwhile \\ & {v2 = nil} \\
		\hline reachability5 & {v1 = n(v2)} \\ & while (v1 $\neq$ nil) do \\ &   v1 := n(v1); \\ &   if (v2 $\neq$ c) {v2 := n(v2)} \\ & endwhile \\ & {n(v2) = nil $\vee$ v2 = c} \\
		\hline reachability6 & {v1 = n(v2)} \\ & while (v1 $\neq$ nil) do \\ & v2 := n(v2) \\ & endwhile \\ & {n(v2) = nil} \\
		\hline
\end{tabular}
\end{table*}

